Optimal Testing for Properties of Distributions

Given samples from an unknown distribution $p$, is it possible to distinguish whether $p$ belongs to some class of distributions $\mathcal{C}$ versus $p$ being far from every distribution in $\mathcal{C}$? This fundamental question has received tremendous attention in statistics, focusing primarily on asymptotic analysis, and more recently in information theory and theoretical computer science, where the emphasis has been on small sample size and computational complexity. Nevertheless, even for basic properties of distributions such as monotonicity, log-concavity, unimodality, independence, and monotone-hazard rate, the optimal sample complexity is unknown. We provide a general approach via which we obtain sample-optimal and computationally efficient testers for all these distribution families. At the core of our approach is an algorithm which solves the following problem: Given samples from an unknown distribution $p$, and a known distribution $q$, are $p$ and $q$ close in $\chi^2$-distance, or far in total variation distance? The optimality of our testers is established by providing matching lower bounds with respect to both $n$ and $\varepsilon$. Finally, a necessary building block for our testers and an important byproduct of our work are the first known computationally efficient proper learners for discrete log-concave and monotone hazard rate distributions.

==> experiments.tex <==
\section{Experimental Evaluation}

In this section, we evaluate the efficacy of our proposed monotonicity tester for $d=1$, and compare it to the estimator proposed in~\cite{BatuKR04}, which we will refer to as the BKR tester henceforth. 
We note that even for $d=1$, our algorithm is seen to outperform the BKR tester in almost all cases. 

Both our algorithm and BKR require a threshold for the test statistic. 
It follows from our results that our estimator's threshold should be at least the standard deviation of the statistic when the distribution is monotone -- this is around $\sqrt{2n}$.
Also, our threshold should be smaller than the expectation of the statistic when the distribution is not in the class.
In particular, we use the value $2\nsmp\eps^2+ \sqrt{2n}$ as the threshold for our test statistic. 

The statistic of BKR imitates an $\ell_2$ test by introducing a discrete statistic that counts the number of collisions within nearby elements.
The argument is that monotone distributions will be locally uniform, and therefore the number of such local collisions should be small. 
They also compare their algorithm with a threshold that is proportional to $O(\log^2 n/\eps)$. However, the constant is not specified in their paper. We considered a few Zipf distributions, which are monotone, and perturbed the probability elements to generate distributions that are $\eps$-far from monotone distributions in total variation distance. We then optimized their threshold for the best possible performance for a range of $n$ and $\eps$. In particular, we came up with the constant of 0.6 for their statistic. Note that one might use uniform distributions, or yet another class of distributions to choose the threshold. 

As is expected, when we run experiments on the class that was used to determine the threshold, the performance of BKR is comparable with our approach for moderate values of $\eps$.
For very small $\eps$, once again their performance degrades, since the number of samples required for concentration of their statistic is proportional to $\eps^{-6}$.
However, for experiments on other monotone classes of distributions (i.e., classes which were not used to train the threshold), our algorithm performed significantly better in almost all cases.
In particular, we also consider a test between the uniform distribution and perturbations thereof (which are guaranteed to be $\ve$-far from monotone).

We give two illustrative plots in the appendix. The number of samples are plotted in logarithmic scale. Both these experiments are run for $n=50,000$. In the uniform case, we take the total variation bound to be $0.05$ and for the Zipf distribution we take it to be $0.07$. As we see for the uniform distribution, our algorithm has accuracy 0.9 with 30000 samples, compared to their accuracy of 0.55. For the Zipf plot, their algorithm is comparable, since we chose the threshold to work the best for this class. 






==> mhr.tex <==
\section{Testing for Monotone Hazard Rate}
\label{sec:MHR}
\gnote{Insert prose}



==> t-modal.tex <==
\section{$t$-modal Distributions}
\label{sec:t-modal}
For a distribution, $\dP$ over $[\absz]$, $i\in[\absz]$ is said to be a \emph{mode} if $\left(p(i)-p(i-1)\right)\cdot \left(p(i+1)-p(i)\right)$ are of different signs. The family of distributions with at most $t$ modes are called $t$-modal distributions. Monotone distributions are 0-modal, and unimodal and 1-modal distribution classes. These classes of distributions are extremely useful to model mixture distributions, for example it is well known that mixture of $t$ Gaussians is a $t$-modal.

PUT SOME RELATED WORK HERE. 

Recently, in a personal communication~\cite{CanonneDGR15} it was shown that testing $t$-modal distributions is possible with $\tilde{O}(t\sqrt{n}/\eps^4)$ samples. Their time complexity is not mentioned explicitly, however we believe there is an implementation in polynomial time. 

Indeed, note that any $t$-modal distribution can be written as a mixture of a $t+1$-mixture of unimodal distributions. Indeed, our results will hold for this more general class of distributions. Since, log-concave and monotone hazard distributions are unimodal, our results also apply to them. 

\subsection{Structural Results} 

We observed that for monotone distributions, there is an oblivious decomposition of the domain, such that the flattening of the underlying distribution over these intervals has a small $\chi^2$ distance. We now extend this argument to $t$-modal distributions. Consider any distribution with at most $t$ modes. Let $b$ be a number, to be decided later. 

Consider a partition of $[\absz]$ into $L\le 1/b+1/t$ intervals such that:
\begin{enumerate}
\item
For each element $i$ with probability at least $1/b$, there is an $I_\ell=\{i\}$.
\item
There are at most two intervals with $\dP(I)\le 1/b$.
\item
Every other interval $I$ satisfies $\dP(I)\in[\frac1b,\frac2b]$.
\end{enumerate}
Let $\dPbar$ be the flattening of $\dP$ over the intervals satisfying these properties.

We first prove our decomposition result for unimodal distributions and then describe appropriate extension to mixtures and more modes. 
Consider any decomposition given as above, and we remove the intervals $I_j$ for which $\dP(I_j)/|I_j|<\frac{\eps}{50\absz}$. This operation essentially removes the tiny probability elements. 
Our key lemma is as follows. 
\begin{lemma}
Let $C>2$. For a unimodal distribution over $[\absz]$, there are at most most $\frac{4\log(50\absz/\eps)}{C\eps}$ intervals $I_j$  satisfy $\frac{\dPj^+}{\dPj^-}<(1+\eps/C)$. 
\end{lemma}
\begin{proof}
To the contrary, if there are more than $\frac{4\log(50\absz/\eps)}{C\eps}$ intervals, then at least half of them are on one side of the mode, however this implies that the ratio of the largest probability and smallest probability is at least $(1+\eps/C)^j$, and if $j>\frac{2\log(50\absz/\eps)}{C\eps}$, is at least $50\absz/\eps$, contradicting that we have removed all such elements. 
\end{proof}

Let $R\ed \frac{4\log(50\absz/\eps)}{C\eps}$ denote the highest number of intervals with large ratios. 
For $A\in [L]$, let $I_A$ denote the subset of intervals with indices in $A$. The following result is now immediate from the previous lemma. 
\begin{lemma}
For any unimodal distribution $\dP$ over $[\absz]$, there is a subset of intervals $I_A$, such that 
\begin{itemize}
\item
$\dP(I_A)>1-\eps/50-2R/b$, and
\item
$\chi^2_{{I_A}}(\dP,\dPbar)\le \eps^2/C^2$.
\end{itemize}
\end{lemma}

Consider the following test. 
\begin{enumerate}
\item
Take $O(b\log b)$ samples to obtain the intervals satisfying the condition above.  
\item
Use $O(b/\eps^2)$ samples obtain a $\dQ$ that is flat over the
intervals of interest. 
\item
If $\dQ$ is at least $\eps/2$ far from the class, output \reject.
\item
Remove all singletons and intervals with $\dQ(I)/|I|<\eps/(50\absz)$. 
\item
\jnote{Remove the intervals with mass at most $1/10b$-- may not be
  necessary}
\item 
Let $\cI_{\rm rem}$ be the remaining intervals
\item
Let $Z_j$ be the $\chi^2$ statistic over the $i$th interval, computed
with $O(\sqrt{\absz}/\eps^2)$ samples. 
\item 
Remove the $R$ largest $Z_j$'s.
\item 
If $\sum_{j}Z_j>\nsmp\eps^2/10$, output \reject.
\item
Output \accept. 
\end{enumerate}

We now prove the accuracy of the algorithm. 
\begin{claim}
If the output $\dQ$ is at most $\eps/2$-far from $\cC$, and $\dP$ is
at least $\eps-$  far from $\cC$, then $\dP$ is at least $\eps/5$-far
from $\dQ$ over the intervals in $\cI_{\rm rem}$. 
\end{claim}
\begin{proof}
Over the singletons, the largest error introduced is at most $\eps/4$
since we take $O(b/\eps^2)$ samples, 
\end{proof}





==> todo.tex <==
\setcounter{section}{-1}
\section{Real Todos}
\begin{itemize}
\item 
\sout{Everything}
\item 
Test previous item
\item
Put in the lower bound derivation from Paninski/PBD's.
\item
$t$-modal distributions -- Think Think Think
\end{itemize}


==> unimodality.tex <==
\section{Testing Unimodality}

One striking feature of Birge's result is that the decomposition of the domain is oblivious to the samples, and therefore to the unknown distribution. However, such an oblivious decomposition will not work for the unimodal distribution, since the mode is unknown. Suppose we know where the mode of the unknown distribution might be, then the problem can be decomposed into monotone functions over two intervals. Therefore, in theory, one can modify the monotonicity testing algorithm by iterating over all the possible $\absz$ modes. Indeed, applying a union bound, it then follows that 
\begin{theorem}(Follows from Monotone)
For $\eps>1/n^{1/4}$, there is an algorithm that takes $O(\frac{\absz^{1/2}}{\eps^2}\log \absz)$ samples, and can test unimodality.  
\end{theorem}

\jnote{It is then easy to extend this to $t$-modal distributions in the most trivial way by taking $t\sqrt{n}/\eps^2$ samples. We dont like it, and will strive for the separation of testing and learning.}.

However, this is not satisfactory since we were only able to prove a lower bound of $\sqrt{\absz}/\eps^2$. In order to overcome the logarithmic barrier introduced by the union bound, we resort to a non-oblivious decomposition of the domain. 

We want to decompose the interval into disjoint intervals such that the probability of each interval is about $O(1/b)$, where $b$ is a parameter, specified later. In particular we consider the following decomposition of  $[\absz]$. 
\begin{enumerate}
\item
For each element $i$ with probability at least $1/b$, there is an $I_\ell=\{i\}$.
\item
There are at most two intervals with $\dP(I)\le 1/{2b}$.
\item
Every other interval $I$ satisfies $\dP(I)\in\left[\frac1{2b},\frac2b\right]$.
\end{enumerate}

Let $I_1, \ldots, I_L$ denote the partition of $[\absz]$ corresponding to these intervals. Note that $L= O(b)$. 
\begin{claim}
There is an algorithm that takes $O(b\log b)$ samples and outputs $I_1, \ldots, I_L$ satisfying the properties above.
\end{claim}

The first step in our algorithm is to estimate the \emph{total probability} within each of these intervals. 
In particular, 
\begin{lemma}
There is an algorithm that takes $m'=O(b\log b/\eps^2)$ samples from a distribution $\dP$, and with probability at least 9/100 outputs a distribution $\dQbar$ that is constant on each $I_L$. Moreover, for any $j$ such that $\dP(I_j)>1/2b$, 
$\dQ(I_j)\in(1\pm\eps)\dQ(I_j)$. 
\end{lemma}
\begin{proof}
Consider any interval $I_j$ with $\dP(I_j)\ge 1/2b$. The number of samples $N_{I_j}$ that fall in that interval is distributed $Binomial(m', \dP(I_j)$. Then by Chernoff bounds for $m'>12 b\log b/\eps^2$, 
\begin{align}
\probof{|N_{I_j}-m'\dP(I_j)|>\eps m'\dP(I_j) }\le& 2\exp\left(\eps^2m'\dP(I_j)/2\right)\\
\le & \frac1{b^2},
\end{align}
where the last inequality uses the fact that $\dP(I_j)\ge 1/2b$. 
\end{proof}

The next step is estimate the distance of $\dQ$ from $UM_{\absz}$. This is possible by a simple dynamic program. If the estimated distance is more than $\eps/2$, we output \reject. 

Our next step is to remove certain intervals. This will be to ensure that when the underlying distribution is unimodal, we are able to estimate the distribution \emph{multiplicatively} over the remaining intervals. 
In particular, we do the following preprocessing step:
\begin{itemize}
\item 
$A= \emptyset$. 
\item 
For interval $I_j$,  
\begin{itemize}
\item 
If \begin{align}
\dQ(I_j) &\notin\left((1-\eps)\cdot\dQ(I_{j+1}),
  (1+\eps)\cdot\dQ(I_{j+1})\right)\ \ \text{ OR }\\
\dQ(I_j) &\notin\left((1-\eps)\cdot\dQ(I_{j-1}), (1+\eps)\cdot\dQ(I_{j-1})\right),
\end{align}
 add $I_j$ to $A$. 
\end{itemize}
\item
Add the (at most 2) intervals with mass at most $1/2b$ to $A$.
\item
Add all intervals $j$ with $\dQ(I_j)/|I_j|<\eps/50n$ to $A$
\end{itemize}

If the distribution is unimodal, we can prove the following about the set of intervals ${A^c}$. 
\begin{lemma}
If $\dP$ is unimodal then, 
\begin{itemize}
\item
$\dP(I_{A^c})\ge 1-\eps/25-1/b - O\left(\log n/(\eps b)\right).$
\item
Except \emph{at most one} interval in ${A^c}$ every other interval $I_j$ satisfies, 
\[
\frac{\dPj^+}{\dPj^-}\le (1+\eps). 
\]
\end{itemize}
\end{lemma}

If this holds, then the $\chi^2$ distance between $\dP$ and $\dQ$ constrained to $A^c$, is at most $\eps^2$. 
This lemma follows from the following result. 
\begin{lemma}
Let $C>2$. For a unimodal distribution over $[\absz]$, there are at most most $\frac{4\log(50\absz/\eps)}{C\eps}$ intervals $I_j$  satisfy $\frac{\dPj^+}{\dPj^-}<(1+\eps/C)$. 
\end{lemma}
\begin{proof}
To the contrary, if there are more than $\frac{4\log(50\absz/\eps)}{C\eps}$ intervals, then at least half of them are on one side of the mode, however this implies that the ratio of the largest probability and smallest probability is at least $(1+\eps/C)^j$, and if $j>\frac{2\log(50\absz/\eps)}{C\eps}$, is at least $50\absz/\eps$, contradicting that we have removed all such elements. 
\end{proof}

We have one additional pre-processing step here. We compute $\dQ(A^c)$ and if it is smaller than $1-\eps/25$, we output \reject. 

Suppose there are $L'$ intervals in $A^c$. Then, except at most one interval in $L'$ we know that the $\chi^2$ distance between $\dP$ and $\dQ$ is at most $\eps^2$ when $\dP$ is unimodal, and the TV distance between $\dP$ and $\dQ$ is at least $\eps/2$ over $A^c$. We propose the following simple modification to take into account, the one interval that might introduce a high $\chi^2$ distance in spite of having a small total variation. If we knew the interval, we can simply remove it and proceed. Since we do not know where the interval lies, we do the following. 

\begin{enumerate}
\item
Let $Z_j$ be the $\chi^2$ statistic over the $i$th interval in $A^c$, computed
with $O(\sqrt{\absz}/\eps^2)$ samples. 
\item 
Let $Z_l$ be the largest among all $Z_j$'s.
\item 
If $\sum_{j, j\ne l}Z_j>\nsmp\eps^2/10$, output \reject.
\item
Output \accept. 
\end{enumerate}

The objective of removing the largest $\chi^2$ statistic is our substitute for not knowing the largest interval. 
We now prove the correctness of this algorithm. 

\paragraph{Case 1 $\dP\in UM_\absz$:} We only concentrate on the final step. The $\chi^2$ statistic over all but one interval are at most $c\cdot m\eps^2$, and the variance is bounded as before. Since we remove the largest statistic, the expected value of the new statistic is \emph{strictly dominated} by that of these intervals. Therefore, the algorithm outputs \accept with at least the same probability as if we removed the spurious interval. 

\paragraph{Case 2 $\dP\notin UM_\absz$:} 
This is the hard case to prove for unimodal distributions. We know that the $\chi^2$ statistic is large in this case, and we therefore have to prove that it remains large even after removing the largest test statistic $Z_l$. 

We invoke Kolmogorov's Maximal Inequality to this end. 
\begin{lemma}[Kolmogorov's Maximal Inequality]
For independent zero mean random variables $X_1,\ldots, X_L$ with finite variance, let $S_\ell=X_1+\ldots X_\ell$. Then for any $\lambda>0$, 
\begin{align}
\probof{\max_{1\le\ell\le L}\left|S_\ell\right|\ge\lambda}\le \frac{1}{\lambda^2}\cdot Var\left(S_L\right). 
\end{align}
\end{lemma}

As a corollary, it follows that $\probof{\max_{\ell}|X_\ell|>2\lambda}\le \frac{1}{\lambda^2}\cdot Var\left(S_L\right)$. 

In the case we are interested in, we let $X_i=Z_\ell-\expectation{Z_\ell}$. Then, similar to the computations before, and the fact that each interval has a small mass, it follows that that the variance of the summation is at most $\expectation{Z_\ell}^2/100$. Taking $\lambda = \expectation{S_L-m\eps^2/3}^2/100$, it follows that the statistic does not fall below to $\sqrt \absz$. 

\begin{theorem}
\label{thm:unimodality}
For $\eps>n^{-1/4}$ samples, there is an algorithm that takes $O(\sqrt{\absz}/\eps^2)$ samples to test unimodality. 
\end{theorem}





